Stroke of Surprise: Progressive Semantic Illusions in Vector Sketching

Visual illusions traditionally rely on spatial manipulations such as multi-view consistency. In this work, we introduce Progressive Semantic Illusions, a novel vector sketching task where a single sketch undergoes a dramatic semantic transformation through the sequential addition of strokes. We present Stroke of Surprise, a generative framework that optimizes vector strokes to satisfy distinct semantic interpretations at different drawing stages. The core challenge lies in the "dual-constraint": initial prefix strokes must form a coherent object (e.g., a duck) while simultaneously serving as the structural foundation for a second concept (e.g., a sheep) upon adding delta strokes. To address this, we propose a sequence-aware joint optimization framework driven by a dual-branch Score Distillation Sampling (SDS) mechanism. Unlike sequential approaches that freeze the initial state, our method dynamically adjusts prefix strokes to discover a "common structural subspace" valid for both targets. Furthermore, we introduce a novel Overlay Loss that enforces spatial complementarity, ensuring structural integration rather than occlusion. Extensive experiments demonstrate that our method significantly outperforms state-of-the-art baselines in recognizability and illusion strength, successfully expanding visual anagrams from the spatial to the temporal dimension. Project page: https://stroke-of-surprise.github.io/

==> 2_related_old.tex <==

\section{Related Work}
\label{sec:related_work}


\paragraph{Generative Vector Graphic Synthesis.}
Early sketch synthesis used category-specific models~\cite{eitz2012humans,jongejan2016quickdraw,sangkloy2016sketchy}. CLIP~\cite{radford2021learning} enabled open-vocabulary generation: CLIPDraw~\cite{frans2022clipdraw} and CLIPasso~\cite{vinker2022clipasso}---extended to scenes~\cite{vinker2023clipascene}---optimize Bézier curves~\cite{bezier1968,decasteljau1959} via differentiable rasterization~\cite{li2020differentiable}, but lack structural guidance. SDS~\cite{poole2022dreamfusion}, built on classifier-free guidance~\cite{ho2022classifier} and latent diffusion~\cite{rombach2022ldm}, provides richer signals. VectorFusion~\cite{jain2023vectorfusion} first applied SDS to SVGs; follow-ups added attention-guided initialization~\cite{xing2023diffsketcher}, semantic decomposition~\cite{xing2024svgdreamer}, neural paths~\cite{zhang2024neuralpath}, dual-domain guidance~\cite{zhao2024dualdomain}, and interactive ideation~\cite{qu2023sketchdreamer}. The objective itself has been refined via variational distillation~\cite{wang2023prolificdreamer}, noise-free objectives~\cite{katzir2023noisefree}, interval score matching~\cite{liang2024luciddreamer}, and reparametrized DDIM~\cite{lukoianov2024ddim}. Other directions bypass optimization via feed-forward inference~\cite{arar2025swiftsketch}, hierarchical modeling~\cite{carlier2020deepsvg}, and autoregressive tokens~\cite{wu2023iconshop,rodriguez2025starvector}, while learned SVG representations~\cite{lopes2019learned} and implicit vector layers~\cite{reddy2021im2vec,thamizharasan2024nivel} improve flexibility---NeuralSVG~\cite{polaczek2025neuralsvg} combines implicit representations with SDS, and SVGFusion~\cite{xing2024svgfusion} operates in a native SVG latent space. Yet all methods treat drawing as a static target. Sequential modeling imposes ordering, but this alone is insufficient when strokes must satisfy two semantic interpretations simultaneously.

% \paragraph{Generative Vector Graphic Synthesis.}
% Early sketch synthesis methods rely on category-specific 
% models trained on large-scale 
% datasets~\cite{eitz2012humans,jongejan2016quickdraw,
% sangkloy2016sketchy}, limiting generalization to unseen 
% concepts. CLIP~\cite{radford2021learning} enabled 
% open-vocabulary generation: CLIPDraw~\cite{frans2022clipdraw} 
% and CLIPasso~\cite{vinker2022clipasso}---later extended to 
% scenes~\cite{vinker2023clipascene}---optimize B\'{e}zier 
% curves~\cite{bezier1968,decasteljau1959} via differentiable 
% rasterization~\cite{li2020differentiable}, yet provide 
% limited structural guidance. Score Distillation 
% Sampling~\cite{poole2022dreamfusion}, built on 
% classifier-free guidance~\cite{ho2022classifier} and latent 
% diffusion models~\cite{rombach2022ldm}, supplies richer 
% gradient signals. VectorFusion~\cite{jain2023vectorfusion} 
% first applied SDS to SVG synthesis; subsequent work refined 
% this along several directions: guiding stroke initialization 
% with diffusion attention maps and introducing augmented 
% SDS~\cite{xing2023diffsketcher}, improving visual quality 
% and diversity through semantic decomposition and 
% particle-based score 
% distillation~\cite{xing2024svgdreamer}, introducing 
% continuous neural path 
% representations~\cite{zhang2024neuralpath}, adopting 
% dual-domain diffusion guidance~\cite{zhao2024dualdomain}, 
% and enabling interactive sketch 
% ideation~\cite{qu2023sketchdreamer}. The distillation 
% objective has also been improved more broadly: variational 
% score distillation increases output 
% diversity~\cite{wang2023prolificdreamer}, noise-free 
% objectives reduce over-smoothing 
% artifacts~\cite{katzir2023noisefree}, interval score 
% matching improves geometric 
% consistency~\cite{liang2024luciddreamer}, and 
% reparametrized DDIM stabilizes the optimization 
% trajectory~\cite{lukoianov2024ddim}. Beyond refining the 
% optimization objective, complementary directions have 
% emerged: feed-forward inference~\cite{arar2025swiftsketch}, 
% hierarchical generative 
% modeling~\cite{carlier2020deepsvg}, and autoregressive 
% token generation~\cite{wu2023iconshop,rodriguez2025starvector} 
% bypass iterative optimization for efficiency; learned SVG 
% representations~\cite{lopes2019learned} and implicit vector 
% layers~\cite{reddy2021im2vec,thamizharasan2024nivel} improve 
% topological flexibility, with 
% NeuralSVG~\cite{polaczek2025neuralsvg} further combining 
% implicit representation with SDS-based optimization, and 
% SVGFusion~\cite{xing2024svgfusion} operating directly in a 
% native SVG latent space. Despite this progress, all 
% existing methods treat the drawing as a static optimization 
% target, leaving the process of stroke accumulation entirely 
% unconstrained. Sequential modeling approaches impose an 
% ordering on this process, yet as we show, this alone is 
% insufficient when strokes must satisfy two semantic 
% interpretations simultaneously.

% \huaish{\paragraph{Text-Guided Vector Sketch Synthesis.}
% Early sketch synthesis methods rely on category-specific recurrent
% models~\cite{ha2017neural} trained on large-scale
% datasets~\cite{eitz2012humans,jongejan2016quickdraw,sangkloy2016sketchy},
% limiting generalization to unseen concepts.
% CLIP~\cite{radford2021learning} enabled open-vocabulary generation:
% CLIPDraw~\cite{frans2022clipdraw} and
% CLIPasso~\cite{vinker2022clipasso}---later extended to
% scenes~\cite{vinker2023clipascene}---optimize
% B\'{e}zier curves~\cite{bezier1968,decasteljau1959} via
% differentiable rasterization~\cite{li2020differentiable},
% yet provide limited structural guidance.
% Score Distillation Sampling (SDS)~\cite{poole2022dreamfusion}, built on
% classifier-free guidance~\cite{ho2022classifier} and latent diffusion
% models~\cite{rombach2022ldm}, supplies richer gradient signals.
% VectorFusion~\cite{jain2023vectorfusion} first applied SDS to SVG
% synthesis, inspiring methods that refine optimization in the latent
% space~\cite{xing2023diffsketcher}, extend to diverse visual styles and
% layered representations~\cite{xing2024svgdreamer}, introduce neural path
% representations~\cite{zhang2024neuralpath}, adopt dual-domain
% diffusion~\cite{zhao2024dualdomain}, and enable text-driven sketch
% ideation~\cite{qu2023sketchdreamer}.
% The distillation objective has been further improved via variational score
% distillation~\cite{wang2023prolificdreamer}, noise-free
% objectives~\cite{katzir2023noisefree}, interval score
% matching~\cite{liang2024luciddreamer}, and reparametrized
% DDIM~\cite{lukoianov2024ddim}.
% More recent work adopts feed-forward
% inference~\cite{arar2025swiftsketch,chen2025svgbuilder} or LLM
% pipelines~\cite{wu2025chat2svg,xing2025llmsvg}, while implicit
% representations~\cite{reddy2021im2vec,thamizharasan2024nivel,
% polaczek2025neuralsvg} and vector-space
% diffusion~\cite{xing2024svgfusion} push quality further.
% Despite this progress, \emph{all} existing methods optimize toward a
% \emph{single} semantic target and impose no constraint on intermediate
% stroke states.
% We build upon SDS as our foundational vehicle but introduce a
% \emph{dual-branch} formulation in which prefix strokes receive
% simultaneous gradients from two competing objectives, discovering a
% shared structural subspace that satisfies both semantic interpretations.
% }



\paragraph{Sequential Sketch Generation.}
Sequential approaches treat drawing as a dynamic process. Recurrent generation via iterative glimpses~\cite{gregor2015draw} laid the foundation; SketchRNN~\cite{ha2017neural} extended this to vector sketches, though LSTM's limited scope restricts complex drawings. Subsequent work added Transformer-based embeddings~\cite{ribeiro2020sketchformer}, self-supervised gestalt learning~\cite{lin2020sketch}, compositional structure~\cite{aksan2020cose}, coarse-to-fine coherence~\cite{bhunia2022doodleformer}, autoregressive Bézier generation~\cite{das2020beziersketch}, diffusion decoders~\cite{wang2023sketchknitter}, sketch completion~\cite{liu2019sketchgan,su2020sketchhealer}, temporal self-supervision~\cite{junior2025temporality}, and hierarchical decomposition~\cite{zang2025hierarchical}. 
Recently, SketchAgent~\cite{vinker2025sketchagent} enables real-time, dialogue-driven stroke generation, while LLM-driven pipelines~\cite{wu2025chat2svg,xing2025llmsvg,chen2025svgbuilder} further improve generation quality and efficiency through feed-forward and hybrid optimization approaches.
Yet all methods greedily commit each stroke to a single semantic target, freezing the prefix once drawn. As our ablation shows (Fig.~\ref{fig:ablation-optimization}), this traps the prefix in a local minimum incompatible with a second concept. Our joint optimization lets prefix strokes shift under dual semantic pressure, finding configurations serving both interpretations.

% \paragraph{Sequential Sketch Generation.}
% Sequential approaches treat drawing as a dynamic generative process. Early work on recurrent image generation through iterative glimpses~\cite{gregor2015draw} established the foundation for this paradigm, which SketchRNN~\cite{ha2017neural} extended to vector sketches by representing each drawing as a sequence of pen motor actions. However, the limited temporal scope of LSTM restricts modeling of complex sketches. Subsequent work addressed this within the sequential formulation: Transformer architectures encode stroke sequences into generalizable embeddings~\cite{ribeiro2020sketchformer} and enable self-supervised learning of sketch gestalt~\cite{lin2020sketch}, compositional embeddings inject explicit part-level structure into the sequence~\cite{aksan2020cose}, coarse-to-fine frameworks improve structural coherence in creative sketch generation~\cite{bhunia2022doodleformer}, autoregressive models generate sketches as sequences of B\'{e}zier curves for scalable vector output~\cite{das2020beziersketch}, diffusion-based decoders improve the realism of generated stroke sequences~\cite{wang2023sketchknitter}, completion models reconstruct sketches from partial inputs~\cite{liu2019sketchgan,su2020sketchhealer}, temporal ordering has been exploited as a self-supervised signal to learn stroke-aware representations~\cite{junior2025temporality}, and hierarchical decomposition scales sequential generation to complex multi-part compositions~\cite{zang2025hierarchical}. Most recently, SketchAgent~\cite{vinker2025sketchagent} and LLM driven pipelines~\cite{wu2025chat2svg,xing2025llmsvg,
% chen2025svgbuilder} generate strokes or components 
% sequentially with real-time visual feedback, approaching human-like drawing behavior. However, all of these methods commit each stroke greedily to a single semantic target, freezing the prefix once drawn. As our ablation shows \ref{fig:ablation-optimization}, this traps the prefix in a local minimum incompatible with a second concept. Our joint optimization instead allows prefix strokes to shift under dual semantic pressure, discovering configurations where a single feature serves both interpretations at once.

% \huaish{\paragraph{Sequential and Agentic Sketch Generation.}
% Unlike synthesis methods that target only the final output, a
% complementary line of research models the \emph{process} of drawing.
% Early recurrent~\cite{ha2017neural} and attention-based
% models~\cite{gregor2015draw} demonstrated that stroke sequences encode
% meaningful structure, and subsequent work deepened this through
% Transformer architectures~\cite{ribeiro2020sketchformer,carlier2020deepsvg,
% bhunia2022doodleformer}, compositional stroke
% embeddings~\cite{aksan2020cose}, B\'{e}zier
% parameterizations~\cite{das2020beziersketch}, and diffusion-based stroke
% generation~\cite{wang2023sketchknitter}.
% Stroke semantics are further explored via reinforcement
% learning~\cite{huang2019paint}, feed-forward neural
% painting~\cite{liu2021painttransformer}, sketch
% completion~\cite{liu2019sketchgan,su2020sketchhealer}, and hierarchical
% generation~\cite{zang2025hierarchical}.
% Most recently, agentic systems such as
% SketchAgent~\cite{vinker2025sketchagent} and LLM-based
% pipelines~\cite{wu2025chat2svg,xing2025llmsvg} generate strokes
% sequentially with real-time visual feedback.
% However, all of these methods commit each stroke \emph{greedily} to a
% single semantic target, freezing the prefix once drawn.
% As our ablation shows (Sec.~4.3, Fig.~10), this traps the prefix in a
% local minimum incompatible with a second concept.
% Our \emph{joint} optimization instead allows prefix strokes to shift
% under dual semantic pressure, discovering configurations where a single
% feature---such as rabbit ears---serves both interpretations at once.
% }



\paragraph{Sketch Perception and Visual Illusions.}
Line drawings' perceptual robustness provides our cognitive foundation. Gestalt closure and figure--ground segregation~\cite{wagemans2012gestalt,wertheimer1923} let viewers complete fragmentary contours~\cite{biederman1987geon,biederman1988surface,kanizsa1979}; even sparse sketches trigger recognition~\cite{cavanagh2005artist,fan2023drawing,singer2023neural,eitz2012humans,yu2017sketchanet}, making them uniquely suited for progressive illusions. Most computational illusion methods exploit \emph{spatial} transformations: shadow art~\cite{mitra2009shadowart}, hybrid images~\cite{oliva2006hybrid}, wire art~\cite{hsiao2018wireart}, and anamorphic distortion~\cite{pratt2023anamorphic,wu2022mirror} or warping~\cite{debnath2025rasp,chang2025lookingglass}. Diffusion-based extensions include Visual Anagrams~\cite{geng2024visualanagrams}, frequency decomposition~\cite{geng2024factorized}, multi-task training~\cite{xu2025anagram}, phase-domain manipulation~\cite{gao2025ptdiffusion}, 3D consistency~\cite{feng2024illusion3d}, fabrication constraints~\cite{burgert2024diffusionillusions}, cross-modal compositing~\cite{chen2024imagessound}, and ambigrams~\cite{zhao2023ambigen}. All require \emph{spatial} manipulation to reveal hidden meaning. We instead introduce \emph{temporal} illusions through progressive stroke accumulation. This asymmetric additive constraint---prefix strokes must be a strict geometric subset of the final drawing---differs fundamentally from symmetric spatial transforms, and is what our dual-branch SDS and Overlay Loss satisfy.

% \paragraph{Sketch Perception and Visual Illusions.}
% The perceptual robustness of line drawings provides the cognitive foundation for our task. Gestalt principles of closure and figure--ground segregation~\cite{wagemans2012gestalt,wertheimer1923} explain how viewers complete fragmentary contours into holistic percepts~\cite{biederman1987geon,biederman1988surface,kanizsa1979}; even a sparse few-stroke drawing can reliably trigger object recognition~\cite{cavanagh2005artist,fan2023drawing,singer2023neural}, a robustness that computational models have demonstrated on standard sketch recognition benchmarks~\cite{eitz2012humans,yu2017sketchanet}. This makes line drawings uniquely suited for progressive illusions: a minimal prefix can unambiguously depict one concept while remaining structurally compatible with a second upon stroke addition. Most computational illusion methods exploit \emph{spatial} transformations to reveal hidden meanings: shadow art encodes shapes viewable only under directional lighting~\cite{mitra2009shadowart}, hybrid images embed two concepts at different spatial frequencies~\cite{oliva2006hybrid}, wire art constructs sculptures readable from multiple viewpoints~\cite{hsiao2018wireart}, and anamorphic methods reveal hidden forms through viewpoint-dependent distortion~\cite{pratt2023anamorphic,wu2022mirror} or geometry-aware warping~\cite{debnath2025rasp,chang2025lookingglass}. Diffusion models have substantially expanded this family: Visual Anagrams~\cite{geng2024visualanagrams} produce multi-view illusions by averaging noise predictions across geometric transforms, an approach extended to perceptual frequency decomposition~\cite{geng2024factorized}, multi-task joint training~\cite{xu2025anagram}, phase-domain manipulation~\cite{gao2025ptdiffusion}, 3D view consistency~\cite{feng2024illusion3d}, physical fabrication constraints~\cite{burgert2024diffusionillusions}, cross-modal compositing~\cite{chen2024imagessound}, and ambigrams~\cite{zhao2023ambigen}. All of these methods require a \emph{spatial} manipulation---a change of viewpoint, orientation, or frequency filter---to reveal the hidden meaning. We instead introduce \emph{temporal} illusions in which semantic transformation arises through progressive stroke accumulation. This asymmetric additive constraint---prefix strokes must constitute a strict geometric subset of the final drawing---is fundamentally different from the symmetric spatial transforms of prior methods, and is precisely what our dual-branch SDS and Overlay Loss are designed to satisfy.

% \huaish{\paragraph{Sketch Perception and Visual Illusions.}
% The perceptual robustness of line drawings provides the cognitive
% foundation for our task.
% Gestalt principles of closure and figure--ground
% segregation~\cite{wagemans2012gestalt,wertheimer1923} explain how
% viewers complete fragmentary contours into holistic
% percepts~\cite{biederman1987geon,biederman1988surface,kanizsa1979};
% even a sparse few-stroke drawing triggers rapid object
% recognition~\cite{cavanagh2005artist,fan2023drawing,singer2023neural},
% a robustness that computational models now match or
% surpass~\cite{eitz2012humans,yu2017sketchanet}.
% This makes line drawings uniquely suited for progressive illusions: a
% minimal prefix can unambiguously depict one concept while remaining
% structurally compatible with a second upon stroke addition.
% Most computational illusion methods exploit \emph{spatial}
% transformations to reveal hidden meanings, including shadow
% art~\cite{mitra2009shadowart}, hybrid images~\cite{oliva2006hybrid},
% wire art~\cite{hsiao2018wireart}, and anamorphic
% sculpture~\cite{pratt2023anamorphic,wu2022mirror,debnath2025rasp,
% chang2025lookingglass}.
% Diffusion models have substantially expanded this family: Visual
% Anagrams~\cite{geng2024visualanagrams} average noise predictions across
% geometric transforms to produce multi-view illusions, an approach
% extended to frequency decomposition~\cite{geng2024factorized},
% multi-task learning~\cite{xu2025anagram}, phase
% transfer~\cite{gao2025ptdiffusion}, 3D
% consistency~\cite{feng2024illusion3d}, shadow
% composition~\cite{luo2025shadowdraw,wang2024neuralshadow}, cross-modal
% compositing~\cite{chen2024imagessound}, physical
% fabrication~\cite{burgert2024diffusionillusions}, and
% ambigrams~\cite{zhao2023ambigen}.
% All of these methods require a \emph{spatial} manipulation---a change
% of viewpoint, orientation, or frequency filter---to reveal the hidden
% meaning.
% We instead introduce \emph{temporal} illusions in which semantic
% transformation arises through progressive stroke accumulation.
% This asymmetric additive constraint---prefix strokes must constitute a
% strict geometric subset of the final drawing---is fundamentally
% different from the symmetric spatial transforms of prior methods, and
% is precisely what our dual-branch SDS and Overlay Loss are designed to
% satisfy.
% }

% \paragraph{Sketch Generation and Sequential Modeling.}
% Vector sketch synthesis evolved from \emph{category-specific} to \emph{open-vocabulary} generation, progressing from edge detection~\cite{canny2009computational, winnemoller2012xdog} and sketch datasets~\cite{ha2017neural, eitz2012humans, sangkloy2016sketchy, jongejan2016quick} through RNNs~\cite{ha2017neural}, Transformers~\cite{ribeiro2020sketchformer, lin2020sketch, carlier2020deepsvg}, GANs~\cite{liu2019sketchgan, ge2020creative}, and autoregressive models~\cite{wu2023iconshop, xu2022deep}. CLIP enabled text-driven synthesis~\cite{frans2022clipdraw, vinker2022clipasso, vinker2023clipascene}, while diffusion-based Score Distillation~\cite{poole2022dreamfusion} was adapted for SVG~\cite{jain2023vectorfusion, xing2023diffsketcher, xing2024svgdreamer, zhang2024text, thamizharasan2024vecfusion, zhao2024vector, qu2023sketchdreamer}, with recent feed-forward~\cite{arar2025swiftsketch, chen2025svgbuilder} and LLM-based methods~\cite{wu2025chat2svg, xing2025empowering, polaczek2025neuralsvg}.
% Stroke ordering encodes semantics, as shown in foundational rendering~\cite{hertzmann1998painterly, hertzmann2003survey} and sequential modeling via attention~\cite{gregor2015draw}, VAEs~\cite{ha2017neural}, embeddings~\cite{aksan2020cose}, completion~\cite{su2020sketchhealer, liu2019sketchgan}, transformers~\cite{bhunia2022doodleformer}, Bézier curves~\cite{das2020beziersketch}, temporality~\cite{junior2025temporality}, and diffusion~\cite{wang2023sketchknitter}. Stroke semantics are explored through RL~\cite{huang2019learning}, optimal transport~\cite{zou2021stylized}, feed-forward~\cite{liu2021paint}, canvas-aware~\cite{hu2023stroke}, style~\cite{shugrina2022neural}, recognizability~\cite{bhunia2020pixelor}, and hierarchical methods~\cite{zang2025generating}. Human-AI collaboration includes co-creative~\cite{davis2015drawing}, turn-taking~\cite{oh2018lead}, creativity~\cite{karimi2020creative}, synchronous~\cite{lawton2023drawing}, and LLM systems~\cite{vinker2025sketchagent, ibarrola2023collaborative}.
% All prior methods target a \emph{single} semantic goal. We introduce \emph{dual-constraint} optimization where prefix strokes forming Object~A are \emph{re-contextualized} into Object~B.




% \paragraph{Sketch Perception and Visual Illusions.}
% Gestalt principles~\cite{wertheimer1923laws, wagemans2012century}, Recognition-by-Components \cite{biederman1987recognition, biederman1988surface}, illusory contours~\cite{kanizsa1979organization}, and cognitive studies~\cite{fan2023drawing, cavanagh2005artist} explain how sparse strokes evoke recognition. Computational approaches surpassed human benchmarks~\cite{eitz2012humans, yu2017sketch} via RL~\cite{muhammad2018learning, muhammad2019goal}, primitives~\cite{alaniz2022abstracting}, implicit~\cite{bandyopadhyay2024sketchinr}, dynamic~\cite{koley2024handle}, grouping~\cite{li2018universal}, saliency~\cite{bhunia2023sketch2saliency}, graphs~\cite{yang2021sketchgnn}, transformers~\cite{wang2024contextseg}, explainability~\cite{qu2023sketchxai}, and neuroscience~\cite{singer2023spatiotemporal}.
% Visual illusions encode multiple meanings via \emph{spatial} transformations: frequency~\cite{oliva2006hybrid}, shadows~\cite{mitra2009shadow}, wire art~\cite{hsiao2018multi}, camouflage~\cite{chu2010camouflage}, evolution~\cite{machado2015evolving}, and morphing~\cite{beier2023feature, alexa2023rigid, seitz1996view}. Diffusion expanded this through view averaging~\cite{geng2024visual}, frequency decomposition~\cite{geng2024factorized}, multi-task~\cite{xu2025diffusion}, phase transfer~\cite{gao2025ptdiffusion}, 3D~\cite{feng2024illusion3d}, fabrication~\cite{burgert2024diffusion}, ambigrams~\cite{zhao2023ambigen}, anamorphic~\cite{chang2025lookingglass, debnath2025rasp}, neural shadows~\cite{wang2024neural}, cross-modal~\cite{chen2024images}, sculpture~\cite{pratt2023bending, wu2022computational}, viewpoint-dependent~\cite{ke2025stealthattack}, biases~\cite{panagopoulou2024evaluating}, and predictive coding~\cite{weilnhammer2017predictive}.
% These rely on \emph{spatial} transformations. We introduce \emph{temporal} concealment where semantics emerge through stroke accumulation.


% \paragraph{Differentiable Rendering and Score Distillation.}
% Bézier foundations~\cite{de1959outillages, bezier1968renault} enabled differentiable rasterization~\cite{li2020differentiable}, improved by splatting~\cite{liu2025b}, ranking~\cite{hirschorn2024optimize}, layers~\cite{ma2022towards}, implicit~\cite{reddy2021im2vec, thamizharasan2024nivel}, latent diffusion~\cite{xing2024svgfusion}, interpolation~\cite{lopes2019learned}, simplification~\cite{simo2016learning}, typography~\cite{iluz2023word}, discrete stylization~\cite{huang2025voxify3d}, and transformation~\cite{wu2019logan}.
% Score Distillation~\cite{poole2022dreamfusion, ho2022classifier} was adapted for vectors~\cite{jain2023vectorfusion, xing2023diffsketcher} and editing~\cite{hertz2023delta}, with improvements via coarse-to-fine~\cite{lin2023magic3d}, variational~\cite{wang2023prolificdreamer}, noise-free~\cite{katzir2023noise}, interval~\cite{liang2024luciddreamer}, DDIM~\cite{lukoianov2024score}, bridge~\cite{mcallister2024rethinking}, collaborative~\cite{kim2023collaborative}, likelihood score matching~\cite{chao2022denoising}, and posterior~\cite{koo2024posterior} formulations. Multi-concept methods use composition~\cite{liu2022compositional}, cross-attention~\cite{kumari2023multi}, neurons~\cite{liu2023cones}, attention~\cite{chefer2023attend}, subject-driven~\cite{ruiz2023dreambooth}, decomposition~\cite{avrahami2023break}, fusion~\cite{gu2023mix}, training-free~\cite{xiao2025fastcomposer}, and guidance~\cite{jiang2025mc}. Multi-view leverages correspondence~\cite{tang2023mvdiffusion}, joint modeling~\cite{liu2023syncdreamer}, hybrid~\cite{bahmani20244d}, satellite-to-ground synthesis~\cite{lee2025skyfall}, and Pareto~\cite{yao2024proud}.
% These focus on \emph{spatial} composition. Our dual-branch SDS addresses \emph{temporal} revelation: prefix strokes receive gradients from both targets, discovering configurations valid for two interpretations.









% \section{Related Work}
% \label{sec:related_work}

% \paragraph{Vector Sketch Generation.}
% Vector sketch generation evolved from \emph{category-specific} to \emph{open-vocabulary} synthesis. Early edge detectors~\cite{canny2009computational, winnemoller2012xdog} motivated learning-based approaches using large-scale datasets~\cite{ha2017neural, eitz2012humans, sangkloy2016sketchy, jongejan2016quick}, progressing through RNNs~\cite{ha2017neural}, Transformers~\cite{ribeiro2020sketchformer, lin2020sketch, carlier2020deepsvg}, GANs~\cite{liu2019sketchgan, ge2020creative}, and autoregressive methods~\cite{wu2023iconshop}, with surveys documenting this evolution~\cite{xu2022deep}.
% Vision-language models enabled open-vocabulary synthesis via CLIP optimization~\cite{frans2022clipdraw}, abstraction control~\cite{vinker2022clipasso}, and scene-level generation~\cite{vinker2023clipascene}. Diffusion approaches applied Score Distillation~\cite{poole2022dreamfusion} to SVG generation~\cite{jain2023vectorfusion} with improvements in initialization~\cite{xing2023diffsketcher}, diversity~\cite{xing2024svgdreamer}, structure~\cite{zhang2024text}, quality~\cite{thamizharasan2024vecfusion, zhao2024vector}, and text-augmented ideation~\cite{qu2023sketchdreamer}. Feed-forward methods achieve faster generation~\cite{arar2025swiftsketch, chen2025svgbuilder}, while LLM-based approaches combine templates with editing~\cite{wu2025chat2svg, xing2025empowering, polaczek2025neuralsvg}.
% All these optimize toward a \emph{single} target. We introduce \emph{dual-constraint} optimization where strokes satisfy two interpretations at different accumulation stages.

% \paragraph{Sequential and Collaborative Sketching.}
% Stroke ordering affects generation and perception. Sequential modeling progressed from spatial attention~\cite{gregor2015draw} through VAEs~\cite{ha2017neural}, compositional embeddings~\cite{aksan2020cose}, completion~\cite{su2020sketchhealer, liu2019sketchgan}, transformers~\cite{bhunia2022doodleformer}, Bézier representations~\cite{das2020beziersketch}, temporality analysis~\cite{junior2025temporality}, and diffusion-based stroke denoising~\cite{wang2023sketchknitter}.
% Stroke-based rendering confirms ordering encodes semantics via reinforcement learning~\cite{huang2019learning}, optimal transport~\cite{zou2021stylized}, feed-forward prediction~\cite{liu2021paint}, canvas-aware methods~\cite{hu2023stroke}, style spaces~\cite{shugrina2022neural}, early recognizability optimization~\cite{bhunia2020pixelor}, and hierarchical generation~\cite{zang2025generating}. Foundational stroke-based rendering~\cite{hertzmann1998painterly, hertzmann2003survey} established the paradigm of image synthesis through ordered brush strokes. Human-AI collaboration spans co-creative agents~\cite{davis2015drawing}, turn-taking~\cite{oh2018lead}, creativity analysis~\cite{karimi2020creative}, synchronous drawing~\cite{lawton2023drawing}, and LLM systems~\cite{vinker2025sketchagent, ibarrola2023collaborative}.
% These share a \emph{coarse-to-fine} paradigm with constant goals. Our \emph{semantic pivot} requires initial strokes forming Object A to be re-contextualized into Object B.

% \paragraph{Sketch Abstraction and Human Perception.}
% Our illusions require understanding which strokes carry semantic weight. Gestalt principles~\cite{wertheimer1923laws, wagemans2012century} explain whole perception from sparse elements. Recognition-by-Components~\cite{biederman1987recognition} shows line drawings match photograph recognition speed~\cite{biederman1988surface}, while illusory contours~\cite{kanizsa1979organization} reveal perceptual completion. Recent cognitive science synthesizes visual abstraction as a core human drawing capacity~\cite{fan2023drawing, cavanagh2005artist}.
% Recognition benchmarks~\cite{eitz2012humans} were surpassed by order-aware networks~\cite{yu2017sketch}. Essential stroke identification uses reinforcement learning~\cite{muhammad2018learning}, goal-driven selection~\cite{muhammad2019goal}, primitive decomposition~\cite{alaniz2022abstracting}, implicit representations~\cite{bandyopadhyay2024sketchinr}, dynamic features~\cite{koley2024handle}, perceptual grouping~\cite{li2018universal}, saliency~\cite{bhunia2023sketch2saliency}, graph segmentation~\cite{yang2021sketchgnn}, transformers~\cite{wang2024contextseg}, and explainability~\cite{qu2023sketchxai}, with neuroscience confirmation~\cite{singer2023spatiotemporal}.

% \paragraph{Computational Visual Illusions.}
% Visual illusions encode multiple meanings through ambiguities. Classic \emph{spatial} approaches include frequency separation~\cite{oliva2006hybrid}, shadow optimization~\cite{mitra2009shadow}, multi-view wire art~\cite{hsiao2018multi}, camouflage images~\cite{chu2010camouflage}, evolutionary methods~\cite{machado2015evolving}, and morphing~\cite{beier2023feature, alexa2023rigid, seitz1996view}.
% Diffusion models expanded capabilities via view averaging~\cite{geng2024visual}, frequency decomposition~\cite{geng2024factorized}, multi-task formulations~\cite{xu2025diffusion}, phase transfer~\cite{gao2025ptdiffusion}, 3D extensions~\cite{feng2024illusion3d}, fabricatable illusions~\cite{burgert2024diffusion}, ambigrams~\cite{zhao2023ambigen}, anamorphic generation~\cite{chang2025lookingglass, debnath2025rasp}, neural shadow art~\cite{wang2024neural}, cross-modal illusions~\cite{chen2024images}, and computational sculpture~\cite{pratt2023bending, wu2022computational}. Studies examine vision-language biases~\cite{panagopoulou2024evaluating} and predictive coding~\cite{weilnhammer2017predictive}.
% These rely on \emph{spatial} transformations. We introduce \emph{temporal} concealment: interpretations emerge through stroke accumulation, requiring prefix strokes valid for both semantics.

% \paragraph{Differentiable Vector Graphics.}
% Foundations trace to de Casteljau~\cite{de1959outillages} and Bézier curves~\cite{bezier1968renault}. Differentiable rasterization~\cite{li2020differentiable} enabled optimization, improved by splatting~\cite{liu2025b} and importance ranking~\cite{hirschorn2024optimize}. Layer-wise addition~\cite{ma2022towards} and implicit representations~\cite{reddy2021im2vec, thamizharasan2024nivel} support progressive generation. Recent advances include latent space diffusion for SVG~\cite{xing2024svgfusion}, latent interpolation~\cite{lopes2019learned}, simplification~\cite{simo2016learning}, typography~\cite{iluz2023word}, and transformation~\cite{wu2019logan}.
% Unlike \emph{single-objective} methods, our \emph{sequence-aware} framework partitions strokes into prefix and delta sets with distinct semantic constraints.

% \paragraph{Score Distillation for 2D Generation.}
% Score Distillation~\cite{poole2022dreamfusion} optimizes representations via diffusion gradients, building on classifier-free guidance~\cite{ho2022classifier}. It was adapted for vectors~\cite{jain2023vectorfusion, xing2023diffsketcher} and editing~\cite{hertz2023delta}. Coarse-to-fine optimization~\cite{lin2023magic3d} improves efficiency. Improvements address quality through variational formulations~\cite{wang2023prolificdreamer}, noise isolation~\cite{katzir2023noise}, interval matching~\cite{liang2024luciddreamer}, reparametrized DDIM~\cite{lukoianov2024score}, bridge-based understanding~\cite{mcallister2024rethinking}, and collaborative distillation~\cite{kim2023collaborative}. Editing uses delta denoising~\cite{hertz2023delta} and posterior distillation~\cite{koo2024posterior}.
% Multi-concept methods employ composition~\cite{liu2022compositional}, cross-attention~\cite{kumari2023multi}, concept neurons~\cite{liu2023cones}, attention manipulation~\cite{chefer2023attend}, subject-driven generation~\cite{ruiz2023dreambooth}, scene decomposition~\cite{avrahami2023break}, efficient fusion~\cite{gu2023mix}, training-free composition~\cite{xiao2025fastcomposer}, and guidance~\cite{jiang2025mc}. Multi-view uses correspondence~\cite{tang2023mvdiffusion}, joint modeling~\cite{liu2023syncdreamer}, and hybrid supervision~\cite{bahmani20244d}. Pareto optimization balances objectives~\cite{yao2024proud}.
% These focus on \emph{spatial} composition. Our dual-branch SDS addresses \emph{temporal} revelation: prefix strokes receive gradients from both targets, discovering configurations valid for both interpretations through accumulation.
